Learning to Localize with Attention: from sparse mmWave channel estimates from a single BS to high accuracy 3D location

One strategy to obtain user location information in a wireless network operating at millimeter wave (mmWave) is based on the exploitation of the geometric relationships between the channel parameters and the user position. These relationships can be built from the line-of-sight (LOS) path and first-order reflections, or purely first-order reflections, requiring high resolution channel estimates to ensure centimeter level accuracy. In this paper, we consider a mmWave multiple-input multiple-output (MIMO) system employing a hybrid architecture, and develop a low complexity two-stage multidimensional orthogonal matching pursuit (MOMP) algorithm suitable for accurate estimation of high dimensional channels. Then, a deep neural network (DNN) called PathNet is designed to classify the order of the estimated channel paths, so that only the LOS path and first-order reflections are selected for localization. Next, a 3D localization strategy exploiting the geometry of the environment is developed to operate in both LOS and non-line-of-sight (NLOS) conditions, while considering the unknown clock offset between the transmitter (TX) and the receiver (RX). Finally, a Transformer based network exploiting attention mechanisms called ChanFormer is proposed to refine the initial position estimate obtained from geometric localization. Simulation results obtained with realistic vehicular channels indicate that localization errors below 28 cm can be achieved for 80% of the users when the LOS path is present, while sub-meter accuracy can be achieved for 55% of the users in NLOS conditions.

==> Sections_old/approach.tex <==
\section{Hybrid model/data driven approach for initial access and localization}\label{sec:HybridApproach}
In this section, we give a thorough description of the algorithms that are implemented in our strategy for joint initial access and localization, in the same order as depicted in Fig. \ref{Sys_model}.


%% Sub-section: explanation of the joint initial access and localization workflow
The diagram of our proposed joint initial access and 3D vehicle localization strategy is shown in Fig. \ref{Sys_model}. First, we collect a number of measurements of mmWave received signals $\bY_M$, and implement MOMP based low complexity channel estimations to acquire $N_{\rm est}$ estimated paths $\hat{\bZ}=[\hat{\bz}_1,...,\hat{\bz}_{N_{\rm est}}]$, where each $\hat{\bz}_l$ contains the estimated channel gains $|\alpha_l|$, \ac{TDoA}s $\tau_l$, \ac{DoA}s ${\boldsymbol\theta}_l$, and \ac{DoD}s ${\boldsymbol\phi}_l$. The proposed localization strategy exploiting path geometric transformations can function in both \ac{LOS} and \ac{NLOS} channels, requiring a sufficient number of 1st order reflections. Due to the majority of the paths being higher order reflections in realistic channels, \textit{PathNet} is offered as a data-driven way to get the path orders and remove the higher order reflections. It predicts the probability of $\hat{\bz}_{l}$ being a LOS component, a 1st reflection, or a higher order reflection, and categorizes the path accordingly. A network like \textit{PathNet} could be the most effective solution for the task given the difficulty in formulating the relationship between the channel parameters and the path orders.  Following that, 3D localization based on two types of geometric transformations can be performed depending on the channel status. We observe that the initial location estimates cannot guarantee sub-meter accuracy for most of the users because of the inherent inaccuracies in the channel estimation and path classification processes.  \textit{ChanFormer} is thus proposed to analyze the relationships among the estimated paths in $\hat{\bZ}$ as well as measure the congruence between the channel features and the initial location estimate $\hat{\bx}_{\rmr}^{\shortparallel}$, and then provide a refined location estimate. The input estimated channel features are extracted through self-attention in the encoder section of the network. These features are then decoded and matched to a more accurate location estimate. The output from \textit{ChanFormer} is a probability map showing which tile contains the true location. Though we use a square tile structure in this paper, the number and the shape of the tiles could be both customized to suit the specific environment

\begin{figure*}[b!]
    \centering
    \includegraphics[width=\textwidth]{Figs/Sys_model.pdf}
    \caption{Diagram of the joint initial access and localization system model. }
    \label{Sys_model}
\end{figure*}
% Sub-section: Communication system model

\subsection{MOMP-based channel estimation}
Conventional compressive channel estimation methods exploit a representation of the received signal based on a dictionary obtained as Kronecker products of the dictionaries for the DoA, DoD, and delay domains. However, in our proposed 3D scenario, using the method will cause a prohibitive computational complexity that modern computers cannot handle. To address the issue, we exploit a sparse representation of the received signal in terms of a product of independent dictionaries instead of a Kronecker product based on MOMP, solving the sparse recovery problems by finding the support of the sparse representation of the channel. Let ${\bf Y}_M\in\mathbb{C}^{N_{\rm q}\times N_{\rmo}}$ be the observation, $\{{\bf \Psi}_{k}\in\mathbb{C}^{N_k^{\rm s}\times N_k^{\rm a}}\ |\ k=1,...,N_{\rmD}\}$ be a collection of $N_{\rm D}$ sparsifying dictionaries, and ${\bf \Phi}\in\mathbb{C}^{N_{\rm q}\times\otimes_{k=1}^{N_{\rm D}}N_k^{\rm s}}$ be the measurement tensor, then the sparse coefficients could be extracted from the tensor ${\bf C}\in\mathbb{C}^{\otimes_{k=1}^{N_{\rm D}}N_k^{\rm s}\times N_{\rm o}}$ by solving the optimization problem:
\begin{equation}\label{eq:MOMP}
	\min_{\bf C}\left(\left\|{\bf Y}_M-\sum_{{\bf i}\in\mathcal{I}}\sum_{{\bf j}\in\mathcal{J}}[{\bf \Phi}]_{:, {\bf i}}\left(\prod_{k = 1}^{N_{\rm D}}[{\bf \Psi}_{k}]_{i_k, j_k}\right)[{\bf C}]_{{\bf j}, :}\right\|^2_{\rmF}\right),
\end{equation}
where $\mathcal{I} = \{{\bf i}=(i_1, \ldots, i_{N_{\rm D}})\in\mathbb{N}^{N_{\rm D}} | i_k \leq N_k^{\rm s}, \ \forall k \leq N_{\rm D}\}$, and $\mathcal{J} = \{{\bf j}=(j_1, \ldots, j_{N_{\rm D}})\in\mathbb{N}^{N_{\rm D}}|j_{d} \leq N_k^{\rm a}, \ \forall k \leq N_{\rm D}\}$.
Intuitively, the fundamental idea of the MOMP method is to rearrange elements into $N_{\rmD}$ orthogonal dimensions and execute tensor multiplications independently along each dimension for large-scale tensors, which yields the same results as using Kronecker product while freeing up more memories to accommodate larger tensor sizes.

The case of $N_{\rmD}=5$ independent dictionaries (for the azimuth and elevation DoA/DoD, and the time domain) is studied in \cite{MOMP2022}, estimating the parameters in the $5$ dimensions simultaneously. For our case, however, to further reduce memory requirements targeting the outdoor localization problem that considers even greater arrays and incredibly fine resolutions, we focus on 1) estimating delays, DoDs, and the equivalent gains that include the effect of the path complex gains and the DoAs ($N_{\rmD}=3$), then 2) retrieving the DoAs from the equivalent gains. Let ${\boldsymbol\Phi}_{m_{\rmr},m_{\rmt}}\in \mathbb{C}^{Q\times N_{\rmt}^{\rmx}\times N_{\rmt}^{\rmy}\times N_{\rmd}}$ be the measurement tensor obtained with $\bF_{m_{\rmt}}$ and $\bW_{m_{\rmr}}$, the whole measurement tensor composed of ${\boldsymbol\Phi}_{m_{\rmr},m_{\rmt}}$ is ${\boldsymbol\Phi}\in \mathbb{C}^{QM_{\rmt} \times N_{\rmt}^{\rmx}\times N_{\rmt}^{\rmy}\times N_{\rmd}}$, and $[{\bf \Phi}]_{Q (m_{\rmt}-1)+q, {\bf i}} = [{\bf F}_{m_{\rmt}}{\bf s}[q-i_3]]_{i_1N_{\rmt}^{\rm x}+i_2}$.
Three independent dictionaries are constructed:
\begin{equation}\label{eq:Dictionaries}
\begin{cases}
    {\bf \Psi}_1 = [\bar{\bf a}_{\rmt}^{\rm x}(\ddot{\phi}_1^{\rm x}), \cdots, \bar{\bf a}_{\rmt}^{\rm x}(\ddot{\phi}_{N_1^{\rm a}}^{\rm x})]\\
	{\bf \Psi}_2 = [\bar{\bf a}_{\rmt}^{\rm y}(\ddot{\phi}_1^{\rm y}), \cdots, \bar{\bf a}_{\rmt}^{\rm y}(\ddot{\phi}_{N_2^{\rm a}}^{\rm y})]\\
	{\bf \Psi}_3 = [{\bp}_{\rmd}(\ddot{t}_1), \cdots, {\bp_{\rmd}}(\ddot{t}_{N_3^{\rm a}})]
 \end{cases},
\end{equation}
where ${\bf \Psi}_1$ and ${\bf \Psi}_2$ are for the discretized azimuth and elevation departure angular domains $\{\ddot{\phi}_1^{\rm x}, \ldots, \ddot{\phi}_{N_1^{\rm a}}^{\rm x}\}$ and $\{\ddot{\phi}_1^{\rm y}, \ldots, \ddot{\phi}_{N_2^{\rm a}}^{\rm y}\}$, and ${\bf \Psi}_3$ is for the discretized delay domain $\{\ddot{t}_1, \ldots, \ddot{t}_{N_3^{\rm a}}\}$, where $[\bp_{\rmd}(\ddot{t})]_{n}=f_{\rmp}\left((n-1)T_s-\ddot{t}\right)$. The effect of combiners and the arrival angular information are inside the equivalent gain tensor ${\bf C}\in\mathbb{C}^{N_{\rm 1}^{\rma}\times N_{\rm 2}^{\rma}\times N_{\rm 3}^{\rma}\times N_s M_{\rmr}}$ which is sparse:
\begin{equation}\label{eq:Coefficients}
	[{\bf C}]_{{\bf j}, :} = \left\lbrace\begin{array}{cl}
		{\boldsymbol \beta}_l^{\transp} & \text{if }\begin{array}{c}
			\phi_l^{\rm x} = \ddot{\phi}_{j_1}^{\rm x}, \phi_l^{\rm y} = \ddot{\phi}_{j_2}^{\rm y},\\
			t_l-t_0 = \ddot{t}_{j_3}
		\end{array};\\
		0 & \text{o.w.}
	\end{array}\right..
\end{equation}
where $[{\boldsymbol \beta}_l]_{N_s (m_{\rmr}-1)+n_s}=\alpha_l[{\bf W}_{m_{\rmr}}]^{*}_{:, n_s}{\bf a}_{\rmr}({\boldsymbol \theta}_l)$. Now the components of Equ. (\ref{eq:MOMP}) are ready, where $\bY_M$ is formed by collecting multiple observations using different pairs of $\bF_{m_{\rmt}}$ and $\bW_{m_{\rmr}}$:
\begin{align}\label{observe_Y}
	\bY_M = \left[\begin{array}{ccc}
		\breve{\bf Y}_{1, 1}& \cdots & \breve{\bf Y}_{M_{\rmr}, 1}\\
		\vdots & \ddots & \vdots\\
		\breve{\bf Y}_{1, M_{\rmt}} & \cdots & \breve{\bf Y}_{M_{\rmr}, M_{\rmt}}\\
	\end{array}\right]\in\mathbb{C}^{QM_{\rmt}\times N_s M_{\rmr}}.
\end{align}

To retrieve the DoA information from the non-zero coefficients of ${\bf C}$ corresponding to the multipath components, the main idea is to correlate the coefficients with angular dictionaries and the DoAs could be determined by where the peaks exist. Let ${\bW}_M = [\breve{\bW}_1, \cdots, \breve{\bW}_{M_{\rmr}}]$, and here we remove the notations for measurement indices for simplicity, ${\boldsymbol \beta}_l$ can be rewritten as ${\boldsymbol \beta}_l = \alpha_l{\bW}_M^{*}{\ba}_{\rmr}({\boldsymbol \theta}_l)$. Hence, assuming every entry of ${\bW}_M$ is orthonormal, multiplying $\boldsymbol\beta_l^*$ to ${\bf W}_M^{*}$ and the angular dictionary gives: 
\begin{equation}
  {\boldsymbol\beta}_l^* {\bW}_M^*{\bf \Psi}_{\rmr}=\alpha_l{\ba}_{\rmr}({\boldsymbol \theta}_l)^{*}{\bW_M\bW^*_M}{\bf \Psi}_{\rmr}=\alpha_l \ba ({\boldsymbol \theta}_l)^*{\bf\Psi}_{\rmr},
\end{equation}
where ${\bf \Psi}_{\rmr}=[{\ba}({\ddot{\boldsymbol \theta}} _1),...,{\ba}({\ddot{\boldsymbol \theta}}_{ N^{\rma}_{4,5}} )]$ is the arrival angular dictionary, which can be constructed as $\bPsi_{\rmr}=\bPsi_4\otimes \bPsi_5$, where  $\bPsi_4$ and $\bPsi_5$ are similar to $\bPsi_1$ and $\bPsi_2$ in Equ. (\ref{eq:Dictionaries}). The DoAs could be thus retrieved referring to the correlation peaks as:
\begin{equation}\label{GetDoA}
\hat{\boldsymbol \theta}_l = \arg\max_{\ddot{\boldsymbol \theta}} \hat{\boldsymbol \beta}_l^*{\bf W}_M^*{\bf\Psi}_{\rmr}.
\end{equation}
Equ. (\ref{GetDoA}) can also be solved using MOMP by independent tensor multiplications in the azimuth and elevation arrival angular domain, especially when $N_4^{\rms}\  (N_5^{\rms})$ is large and high resolutions are needed. The computational complexity of our channel estimation algorithm is:
\begin{equation}
\begin{aligned}
    \cO(& N_{\rm est}(QM_{\rmt}+N_sM_{\rmr})(\sum_{k=1}^3 N_k^{\rma} N_k^{\rms})\\
&+N_{\rm est}N_s M_{\rmr}(N_4^{\rma} N_4^{\rms}+N_5^{\rma} N_5^{\rms})),
\end{aligned}
\end{equation}
which is significantly lower than that of using the original OMP algorithm -- $\cO\left(N_{\rm est}(QM_{\rmt}+N_sM_{\rmr})(\prod_{k=1}^5 N_k^{\rma} N_k^{\rms}) \right)$ -- that modern computers cannot handle for our 3D settings.

The channel parameters required for localization -- 3D DoDs/DoAs and TDoAs -- are now available, except the path order which determines whether to discard an estimated path or not, as only LOS and 1st order reflections are usable in our system. The path classification problem is addressed in Sec. \ref{approach_path_class}.

\begin{figure}[t!]
    \centering
    \includegraphics[width=.9\columnwidth]{Figs/correlate.pdf}
    \caption{Correlation between each two of the channel parameters.}
    \label{CorrChanParam}
\end{figure}
\begin{figure}[t!]
	\centering
	\includegraphics[width=.9\columnwidth]{Figs/PathNet.pdf}
	\caption{Architecture of \textit{PathNet}.}
	\label{classify_DNN_arch}
\end{figure}
\begin{figure*}[t!]
	\centering
	% \column
\subfloat[]{%
		\label{DoD_illustration}
		\includegraphics[height=0.22\textwidth]{Figs/DoD_illustration.pdf}}
	\subfloat[]{%
		\label{LOSNLOS_loc_model}
		\includegraphics[height=0.22\textwidth]{Figs/LOSNLOS_loc_model.pdf}}
	\subfloat[]{%
		\label{NLOSOnly_loc_model}
		\includegraphics[height=0.22\textwidth]{Figs/NLOSOnly_loc_model.pdf}}
	\caption{(a) Illustration of DoD, of which the unitary vector ${\boldsymbol \phi}=[\cos\phi^{\rmy}\cos\phi^{\rmx}, \cos\phi^{\rmy}\sin\phi^{\rmx}, \sin\phi^{\rmy}]^{\transp}$; (b) LOS+NLOS localization; (c) NLOS-only localization. }
	\label{loc_model}
\end{figure*}
\subsection{\textit{PathNet} for path classification}\label{approach_path_class}
The geometric relationships regarding LOS or NLOS channels can be exploited as shown in Fig. \ref{loc_model} for vehicle localizations. We consider the LOS path and/or a sufficient number of 1st order reflections necessary for our scheme, and higher order paths should be discarded. It is difficult to describe the relationship between the path order and the path parameters using a well-formulated model, thus we employ a data-driven approach based on DL to learn the relationship. To build a reasonable network, the correlations between the channel parameters and the path order are studied. As shown in Fig. \ref{CorrChanParam}, the path gain $|\alpha|$, TDoA $\tau$, azimuth and elevation DoAs/DoDs $\theta^{\rmx}$, $\theta^{\rmy}$, $\phi^{\rmx}$, $\phi^{\rmy}$ contribute to the path order, except the phase. Therefore, we decide the input of the network to be the normalized version of these parameters, denoted as $\bz=[|\alpha|^2, \tau, \theta^{\rmx}, \theta^{\rmy}, \phi^{\rmx}, \phi^{\rmy}]$. Every estimated path $\hat{\bz}_l$ must fall into one of the three categories: LOS ($c=1$), 1st order reflections ($c=2$), or others ($c=3$), given the probability vector output from \textit{PathNet}, which is defined as:
\begin{equation}
    \bp(c|\hat{\bz}) = \mathcal{F}(|\alpha|^2, \tau, \theta^{\rmx}, \theta^{\rmy}, \phi^{\rmx}, \phi^{\rmy}; {\boldsymbol\mu}),
\end{equation}
where $[\bp(c|\hat{\bz})]_{i}=p(c=i|\hat{\bz},i\in\{1, 2, 3\})$, $\mathcal{F}(\cdot)$ represents the operations performed by \textit{PathNet}, and ${\boldsymbol\mu}$ represents the network parameters to be trained. Hence, among $N_{\rm est} $ estimated paths of a channel, the LOS and 1st order reflections can be identified according to:
\begin{equation}
    \hat{c}(\hat{\bz}) = \arg\max\limits_{i\in\{1,2,3\}}p(c=i|\hat{\bz}).
\end{equation}
As the input parameters are not like images with visible local features or like \ac{NLP} problems that are usually context-sensitive and involving historical information, we simply adopt \ac{FC} layers as the major components of the network, as it is usually a cheap way of learning non-linear combinations of features embedded in the input. The proposed architecture is shown in Fig. \ref{classify_DNN_arch}. To select an effective loss function to train the network, we notice that more penalties need to be applied when classifying the higher order as LOS/1st order reflections, which ruins the localization derivations, whereas less penalties make sense when the opposite happens because there are times when it is even advantageous to remove the LOS/1st order reflections with the features closer to those of higher order reflections, which may indicate inaccurate channel estimates. As such, a weighted cross entropy loss instead of a regular cross-entropy loss is adopted to adjust the penalties:
\begin{equation}
    \mathcal{L}({\boldsymbol\mu})=-e^{-\eta (c({\bf z})-\hat{c}({\bf z}))}\cdot [\bp(c|\bz)]_{c(\bz)},
\end{equation}
where $\eta$ is the customized weight coefficient.

\subsection{Localization via geometric transformations}
Assuming imperfect synchronization between the vehicle and BS, and the clock offset to be $t_0$, two geometric transformations depending on the channel state are presented in Fig. \ref{LOSNLOS_loc_model} and \ref{NLOSOnly_loc_model}. 

\textbf{LOS+NLOS:} Taking the example of LOS and a single 1st reflection ($l=1$) for the LOS+NLOS case as shown in Fig. \ref{LOSNLOS_loc_model}, the angle between the DoAs of the two paths is defined as $\dot{\theta}=\arccos({\boldsymbol \theta}_{\rm LOS}^{\transp}{\boldsymbol \theta}_l)$, and similarly $\dot{\phi}_l=\arccos({\boldsymbol \phi}_{\rm LOS}^{\transp}{\boldsymbol \phi}_l)$ represents the angle between the DoDs. The geometric transformation of the paths based on the law of sines can be acquired as:
\begin{equation}\label{sin_law}
    \frac{d_{\rm LOS}}{\sin(\dot{\theta}_l+\dot{\phi}_l)}=\frac{d_l^{\rm D}}{\sin(\dot{\theta}_l)}=\frac{d_l^{\rm A}}{\sin(\dot{\phi}_l)},
\end{equation}
where $d_{\rm LOS}=||{ \rm \bx}_{\rmt}-{\rm \bx}_{\rmr}||$ is the straight line distance between the 3D positions of the TX ${ \rm \bx}_{\rmt}$ and RX ${\rm \bx}_{\rmr}$, which can be calculated by $d_{\rm LOS}=v_{\rmc}t_{\rm LOS}$, where $v_{\rmc}$ is the light speed and $t_{\rm LOS}$ is the time light travels; $d_l^{\rm D}$ ($d_l^{\rm A}$) is the distance between the TX (RX) and the interaction point on any surface, so that $d_l^{\rm D}+d_l^{\rm A}=v_{\rmc}t_l$. Hereby we have:
\begin{equation}\label{DDoF}
    d_l^{\rmD}+ d_l^{\rmA}-d_{\rm LOS} = v_{\rmc}(t_l-t_{\rm LOS}) = v_{\rmc}\tau_l,
\end{equation}
where $\tau_l$ is the TDoA between the 1st reflection $l$ and the LOS. Combining Equ. (\ref{sin_law}) and (\ref{DDoF}), $d_{\rm LOS}$ can be derived as:
\begin{equation}
    \hat{d}_{\rm LOS} =\frac{v_{\rmc}\tau_l \sin(\dot{\theta}_l + \dot{\phi}_l)}{\sin(\dot{\theta}_l)+ \sin(\dot{\phi}_l)-\sin(\dot{\theta}_l + \dot{\phi}_l)}.
\end{equation}
When the number of estimated 1st order reflections $L_{c=2}\geq 1$, $\hat{d}_{\rm LOS}$ can be obtained by solving the \ac{LS} estimation problem:
{\small
\begin{equation}
    \hat{d}_{\rm LOS} =\frac{<v_{\rmc}\cdot{{\rm{\boldsymbol\tau}}} \odot\sin(\dot{\boldsymbol \theta} + \dot{\boldsymbol \phi}), \sin(\dot{\boldsymbol \theta})+ \sin(\dot{\boldsymbol \phi})-\sin(\dot{\boldsymbol \theta} + \dot{\boldsymbol \phi})>}{\|\sin(\dot{\boldsymbol \theta})+ \sin(\dot{\boldsymbol \phi})-\sin(\dot{\boldsymbol \theta} + \dot{\boldsymbol \phi})\|^2},
\end{equation}
}
where ${\boldsymbol\tau}=[\tau_1,...,\tau_{L_{c=2}}]^{\transp}$, $\dot{\boldsymbol\theta}=[\dot{\theta}_1,...,\dot{\theta}_{L_{c=2}}]^{\transp}$, and $\dot{\boldsymbol\phi}=[\dot{\phi}_1,...,\dot{\phi}_{L_{c=2}}]^{\transp}$.
Finally, the vehicle location could be determined by:
\begin{equation}
    \hat{\rm\bx}_{\rmr}={\rm\bx}_{\rmt}+ \hat{d}_{\rm LOS}\cdot{\boldsymbol\phi}_{\rm LOS}.
\end{equation}

\textbf{NLOS-Only: }As shown in Fig. \ref{NLOSOnly_loc_model}, the geometric transformation for path $l$ could be formed with an extension of Equ. (\ref{DDoF}):
\begin{equation}\label{NLoS_loc_equ}
\begin{cases}
{\bf x}_{\rmr}+{\boldsymbol \theta}_l d_l^{\rmA} = {\bx}_{\rmt} +{\boldsymbol \phi}_l d_l^{\rmD}\\
d_l^{\rm A}+d_l^{\rmD}=\Delta d_l+d_0
\end{cases},
\end{equation}
where $\Delta d_l=v_{\rmc}(t_l-t_0)$, and $d_0=v_{\rmc}t_0$. The vehicle location can be rewritten as:
\begin{equation}\label{NLOS_geo}
    \bx_{\rmr}=\bx_{\rmt}+({\boldsymbol\phi}_l+{\boldsymbol\theta}_l)d_l^{\rmD}-{\boldsymbol\theta}_l(\Delta d_l+d_0),
\end{equation}
and $d_l^{\rmD}$ is estimated as:
\begin{equation}\label{NLOS_dD}
    \hat{d}_l^{\rmD}=\frac{<{\boldsymbol\phi}_l+{\boldsymbol\theta}_l, \bx_{\rmr}- \bx_{\rmt}+{\boldsymbol\theta}_l(\Delta d_l+d_0)>}{ ||{\boldsymbol\phi}_l+{\boldsymbol\theta}_l||^2}.
\end{equation}
Substitute $d_l^{\rmD}$ in Equ. (\ref{NLOS_geo}) with the expression in Equ. (\ref{NLOS_dD}), and let  $\Theta_l=\frac{({\boldsymbol \theta}_l+{\boldsymbol \phi}_l)({\boldsymbol \theta}_l+{\boldsymbol \phi}_l)^{\transp}}{||{\boldsymbol \theta}_l+{\boldsymbol \phi}_l||^2}$:
\begin{equation}
    \bx_{\rmr}=(\bI-\Theta_l)\bx_{\rmt}+\Theta_l\bx_{\rmr}-(\bI-\Theta_l){\boldsymbol\theta}_l(\Delta d_l+d_0),
\end{equation}
which could be reduced to:
\begin{equation}\label{NLOS_solve_formu}
    \begin{aligned}(\bI-\Theta_l)(\bx_{\rmr}+{\boldsymbol\theta}_l d_0)=(\bI-\Theta_l)[\bI,{\boldsymbol\theta}_l][\bx_{\rmr};d_0]\\ =(\bI-\Theta_l)(\bx_{\rmt}-{\boldsymbol\theta}_l \Delta d_l)\end{aligned}.
\end{equation}
The rank of $\Theta_l$ being $1$ makes the rank of $(\bI-\Theta_l)$ to be $3-1=2$, and the rank of $[\bI,{\boldsymbol\theta}_l]$ is $3$, so the rank of $(\bI-\Theta)[\bI,{\boldsymbol\theta}_l]$ is $\min\{2,3\}=2$. When only a single 1st reflection is available, the solution set of Equ. (\ref{NLOS_solve_formu}) with $4$ unknowns  --  3D vehicle position $\bx_{\rmr}$ and the clock offset $t_0$ -- has a dimension of $4-2=2$. Hence, there must be at least $3$ estimated 1st order reflections for the problem to have a unique solution of $[\bx_{\rmr};d_0]$, which can be solved using \ac{LS} estimation as:
\begin{equation}\label{eq:final_loc}
[\hat{\bf x}_{\rmr};\hat{d}_0] = {\bf A}^{-1}{\bf b},
\end{equation}
for 
$$
\begin{cases}
{\bf A} = \sum_{l=1}^{L_{c=2}}[\bI,{\boldsymbol \theta}_l]^{\transp}(\bI -\Theta_l)[\bI,{\boldsymbol \theta}_l]\\ 
{\bf b} = \sum_{l=1}^{L_{c=2}}[\bI,{\boldsymbol \theta}_l]^{\transp}(\bI-\Theta_l)({\bf x}_{\rmt}-{\boldsymbol \theta}_l\Delta d_l)
\end{cases}.
$$
Once $\hat{\bf x}_{\rmr}$ is obtained, we can use the information to determine the location of the reflection points as well by inputting $\hat{\bf x}_{\rmr}$ into Equ. (\ref{NLoS_loc_equ}).

For both the LOS+NLOS and NLOS-only situations, multiple combinations of paths could exist to yield differing location estimates. In such a case, iterating over various combinations of paths and removing illogical localization results, e.g., those with unrealistic height estimations $\hat{x}_{\rmr}^{\perp}=[\hat{\bx}_{\rmr}]_3$ (assuming height information is acquirable as downlink channel estimation is performed), can lead to satisfactory localization results. In the vehicular setting, we care particularly about the 2D location estimate $\hat{\bx}_{\rmr}^{\shortparallel}=[\hat{\bx}_{\rmr}]_{:2}$, which is the XY-plane location vector, for performance evaluations in the following sections.

%% sub-section: "ChanFormer" for localization refinement
\begin{figure}[t!]
	\centering
	% \column
	\subfloat[]{%
		\label{tile_structure}
		\includegraphics[width=0.6\columnwidth]{Figs/tile_struct.pdf}}\\
	\subfloat[]{%
		\label{distance_prob_model}
		\includegraphics[width=0.75\columnwidth]{Figs/distance_prob_model.pdf}}
	\caption{Illustration of (a) a $N_g\times N_g=3\times 3$ tile structure; (b) $p(\widetilde{\bx}_{\rmr}^{\shortparallel}|\hat{\bZ})$ \textit{vs.} $\epsilon(\widetilde{\bx}_{\rmr}^{\shortparallel})$ under various $\gamma$ and $\delta$ settings.}
	\label{fig_dist_prob_model}
\end{figure}
\subsection{ChanFormer for localization refinement}
Noises may be introduced throughout the channel estimation and path classification process, and errors that accumulate and propagate will have a detrimental impact on the localization results. Modeling the noise is impractical as there are numerous influential factors, thus we turn to DL to approximate the mapping between the estimated paths and the true location. Instead of directly predicting the vehicle location from the received signal, where the localization accuracy is usually compromised in outdoor scenarios, we consider a $N_g\times N_g$ tile structure with a specified grid size $g_s$ around the initial 2D location estimate $\hat{\bx}^{\shortparallel}_{\rmr}$, as an example shown in Fig. \ref{tile_structure}, and create a network called \textit{ChanFormer} that provides the probability of a tile containing the true location:
\begin{equation}
p\left(\widetilde{\bx}_{\rmr}^{\shortparallel}|\hat{\bZ}\right)=p\left(\bx_{\rmr}^{\shortparallel}=\widetilde{\bx}_{\rmr}^{\shortparallel}|\hat{\bZ}, \widetilde{\bx}_{\rmr}^{\shortparallel}=\hat{\bx}^{\shortparallel}_{\rmr}+[n_{\rmx}g_s, n_{\rmy}g_s]^{\transp}\right),
\end{equation}
where $\hat{\bZ}=[\hat{\bz}_1;...;\hat{\bz}_{N_{\rm est}}]$ is the estimated channel containing $N_{\rm est}$ estimated paths, and $|n_{\rmx}|,|n_{\rmy}|\in\left\{0,1,...,\frac{N_g-1}{2}\right\}$. $p(\widetilde{\bx}_{\rmr}^{\shortparallel}|\hat{\bZ})$ should be negatively related to the distance between $\widetilde{\bx}_{\rmr}^{\shortparallel}$ and $\bx_{\rmr}^{\shortparallel}$, which is formulated as :
\begin{equation}\label{dist_prob_model}
    p\left(\widetilde{\bx}_{\rmr}^{\shortparallel}|\hat{\bZ}\right)=\frac{1}{1+e^{-\gamma\left(1-\frac{||\widetilde{\bx}_{\rmr}^{\shortparallel}-\bx_{\rmr}^{\shortparallel}||}{\delta}\right)}},
\end{equation}
where $\gamma$ is the belief factor, and $\delta$ is the scale factor for the distance $\epsilon(\widetilde{\bx}_{\rmr}^{\shortparallel})=||\widetilde{\bx}_{\rmr}^{\shortparallel}-\bx_{\rmr}^{\shortparallel}||$. An illustration of the effects of $\gamma$ and $\delta$ can be found in Fig. \ref{distance_prob_model}. \textit{ChanFormer} is meant to analyze $\hat{\bx}^{\shortparallel}_{\rmr}$ and its surroundings $\widetilde{\bx}_{\rmr}^{\shortparallel}$ to find the one that most likely meets the current estimated channel condition, i.e., $\max_{\widetilde{\bx}_{\rmr}^{\shortparallel}}p(\hat{\bZ}|\widetilde{\bx}_{\rmr}^{\shortparallel})$. The entire network can be formulated as:
\begin{equation}
    \hat{\bP}\left(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel}\right)=\mathcal{T}\left(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel}; {\boldsymbol\omega}\right)\in \mathbb{R}^{1\times N_g^2},
\end{equation} 
where $\boldsymbol\omega$ is the network parameters to be trained. Inspired by the idea of the original \textit{Transformer} \cite{Transformer2017}, the core concept of \textit{ChanFormer} is an encoder for \textit{Self-Attention} to extract features of the input estimated channel $\hat{\bZ}$, and a decoder to analyze the relationships between the estimated channel features and the initial location estimate $\hat{\bx}_{\rmr}^{\shortparallel}$ using \textit{Encoder-Decoder Attention}. The proposed architecture is shown in Fig. \ref{ChanFormer}.
\begin{figure*}[!h]
    \centering
    \includegraphics[width=\textwidth]{Figs/ChanFormer.pdf}
    \caption{Architecture of \textit{ChanFormer}. The self-attention block extracts the intra and crossover features of the input estimated paths; The encoder-decoder block analyzes the relationship between the initial location estimate and the extracted features of the estimated paths. }
    \label{ChanFormer}
\end{figure*}

\textbf{Encoder: }The workflow starts with \ac{FC} layers embedding the input estimated paths to vectors with a length of $256$. Then, the self-attention process begins by creating three abstraction matrices -- \textit{query}, \textit{key}, and \textit{value} matrices, denoted as $\bQ$, $\bK$, and $\bV$ respectively, where each row of the matrices corresponds to an estimated path. Conceptually, each $\hat{\bz}_l$ now has a high-dimensional interpretation of its features in its \textit{value} $[\bV]_{l,:}$, which can be indexed by its \textit{key} $[\bK]_{l,:}$. The following attention layer then evaluates the relationships among the paths by:
\begin{equation}
    {\rm Attention}(\bQ, \bK, \bV)={\rm softmax}\left(\frac{\bQ\bK^{\transp}}{\sqrt{d_{\rmk}}}\right)\bV,
\end{equation}
where $d_{\rmk}$ is the dimension of $[\bK]_{l, :}$, and $\rm softmax$ is for atoms along $\rm axis=2$. The softmax score determines how much true channel information is represented by the $l$-th estimated path by examining the correlation between $\hat{\bz}_l$ and all the paths in $\hat{\bZ}$. It is expected that $\hat{\bz}_l$ will have the highest softmax score with itself, but other paths that have quite accurate estimations will also be assigned a relatively high score. Therefore, the $\rm Attention$ output is the expression of each path that integrates information from all other paths. The less reliable estimated paths will have a smaller influence on the expressions. Simply put, this means that the attention mechanism places more emphasis on the more accurate paths in this step, so that the true channel is better represented, regardless of the presence of the noises from the channel estimation process and/or the misclassified paths. In addition, the attention layer is capable of analyzing the input without being constrained by its chronicle orders, which exceeds the capabilities of the convolutional layer that considers path relationships within a fixed window, or the \ac{FC} layer that relies on connections of all the input parameters.

\textbf{Decoder: }The input $\hat{\bx}_{\rmr}^{\shortparallel}$ serves as a \textit{query}, referring to which the network generates the probability map $\bP(\hat{\bZ})^{\star}\in \mathbb{R}^{N_g\times N_g}$ of the tiles with $\hat{\bx}_{\rmr}^{\shortparallel}$ at the center. Note that, though $\hat{\bx}_{\rmr}^{\shortparallel}$ is the only input at the decoder, the network actually takes all the candidate locations in the tiles into consideration. In this part, the attention layer improves the initial location estimate accuracy by assigning a higher probability to a candidate location $\widetilde{\bx}_{\rmr}^{\shortparallel}$ that aligns better with the channel representation obtained from the encoder. Note that the output $\hat{\bP}(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})$ is reshaped to $\bP(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})^{\star}\in\mathbb{R}^{N_g\times N_g}$ to acquire the probability map to simplify the process of accessing $\widetilde{\bx}_{\rmr}^{\shortparallel}$ associated with $p(\widetilde{\bx}_{\rmr}^{\shortparallel}|\hat{\bZ})$. By referring to the tile with the highest probability:
\begin{equation}
\begin{aligned}
[j^{\star}, i^{\star}] &= \arg\max\limits_{j, i}\left[\hat{\bP}(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})^{\star}\right]_{j,i}
\Rightarrow\\ &[n_{\rmx}^{\star}, n_{\rmy}^{\star}]=\left[i^{\star}-\frac{N_g+1}{2}, \frac{N_g+1}{2}-j^{\star}\right],
\end{aligned}
\end{equation}
the refined location is given by:
\begin{equation}
    \widetilde{\bx}_{\rmr}^{\shortparallel(\star)}=\hat{\bx}^{\shortparallel}+[n_{\rmx}^{\star}g_s, n_{\rmy}^{\star}g_s]^{\transp}.
\end{equation}

To train the network, MSE loss or the \ac{KL} divergence loss to learn the probability map distribution could be used.



==> Sections_old/conclusion.tex <==
\section{Conclusion and Future Work}\label{conclu}
We used a hybrid data/model driven method to realize 3D localization in the mmWave V2I network. We considered a realistic channel model that includes the filtering effects and an unknown TX-RX clock offset, and generated channel datasets using ray-tracing. We proposed to first remove the high order reflections -- which are the majority of a realistic channel -- using \textit{PathNet}, which achieved a classification accuracy of $99\%$ that provided a solid foundation for the localization strategy. The model-driven 3D location estimator is then formulated through geometric transformations among the locations of the vehicle, scatters, and the RSU. The estimator worked in both LOS and NLOS scenarios, requiring sufficient 1st order reflections though. The estimator realized sub-meter accuracies for $80\%$ of users in LOS channels and for $35\%$ of users in NLOS channels. We treated the results to be less satisfactory, and thus designed the location refinement network \textit{ChanFormer}, which found a better representation of an estimated channel and indicated the most probable vehicle location under the channel status. As a result, $95\%$ of users in the LOS channels can have a 2D localization accuracy of $0.45$ m, and $50\%$ of users in the NLOS channels can have an accuracy of $0.75$ m. Overall, the performance has been improved by $55\%\sim 65\%$ depending on the scenario. The results demonstrate that the idea of attention is well-suited to our scenario without any gaps, and also highlight the potential of migrating advanced DNN architectures to the field of wireless communications. 

Current work is for initial access, where the NLOS-only situation could be a bit concerning regarding the achieved accuracy. Integrating other onboard sensors could be a solution for higher accuracy. In addition, this research will be extended to vehicle location tracking using mmWave RX signals or sensor fusion. With historical channel and location information, solutions for occasional blockages in a trajectory could be provided. Attention based methods could also be used, which could outperform traditional network architectures for time series processing, e.g., \ac{LSTM} \cite{van2020review}, which processes the inputs sequentially and can be still prone to losing important earlier information due to memory limitations. Furthermore, in highly dynamic scenarios, an alternative approach to consider is \ac{V2V} sidelink assisted localization, which facilitates direct communication between vehicles without relying on connectivity through cellular infrastructures.


==> Sections_old/prior_work.tex <==
\subsection{Prior work}\label{PriorWork}
% channel est  
The foundation of our work is the mmWave channel estimation for initial access considering realistic channels. Existing methods often exploit the sparse nature of mmWave \ac{MIMO} channels and rely on \ac{CS} to solve the sparse recovery problem \cite{Wu2019, gurbuz2018sparse, mejri2020structured, SWOMP2018, Coma2018, Venugopal2017}. Variations of the \ac{OMP} algorithm are used for adaptive and accurate channel estimations. A low-complexity \ac{OMP} algorithm exploiting the inherent correlation in the signal angular domain and scattering information is proposed in \cite{Wu2019}, and a parameter perturbed \ac{OMP} algorithm which jointly solves the unknown mmWave channel itself as well as the basis mismatch due to the off-the-grid problem is proposed in \cite{gurbuz2018sparse}. While only narrow bands and frequency-flat channels are considered in \cite{Wu2019, gurbuz2018sparse}, \cite{mejri2020structured, SWOMP2018, Coma2018, Venugopal2017} offer solutions for wideband frequency-selective mmWave channels. The simultaneous \ac{OMP} (SOMP) algorithm \cite{tropp2005simultaneous} is the core for \cite{mejri2020structured, SWOMP2018 }. In \cite{mejri2020structured}, a joint subcarrier-block-based scheme is proposed using continually distributed angles of arrival and departure, while in \cite{SWOMP2018}, simultaneous weighted \ac{OMP} (SWOMP) is presented which generalizes the SOMP algorithm to account for the correlated noise after combining. In \cite{Coma2018}, the authors focus on compressive channel estimation on the uplink to configure precoders/combiners for the downlink based on channel reciprocity and develop two algorithms for both purely digital and hybrid architectures. In \cite{gao2022deep, liu2021sparsity, ma2020sparse}, \ac{DL} methods are investigated, including a 3D \ac{CNN} that approximates the sparse Bayesian learning process \cite{gao2022deep}, a concatenated block architecture based on \ac{CNN} for extracting the channel coefficients \cite{liu2021sparsity}, and a \ac{FC} network for beamspace channel amplitude estimation and channel reconstruction \cite{ma2020sparse}. Channel models in these \ac{DL} methods are simplified without filtering effects, and the combining process is omitted in \cite{liu2021sparsity, ma2020sparse}. All the above methods are carried out in the frequency domain without estimating the delays, which is not suitable for our localization strategy which depends on the delay for the calculation of light traveling distance to form the equations of geometric transformations.   Researchers in \cite{Venugopal2017} have provided channel estimation techniques for purely time or frequency domains, however, implementing the algorithm in our 3D outdoor setting with high dictionary resolutions for precise localization will cause an excessively high complexity, which grows exponentially with the dimension of the signal. In addition, these algorithms capable of estimating the dominant paths can be adequate for communication purposes but may fall short for localization, as a sufficient number of reflections are required. 

There is existing research on joint mmWave channel estimation and vehicle localization. Single-shot localization \cite{Talvitie2019,  Jiang2021, Zhu2019} can be realized through two-stage approaches, which involve channel estimation followed by relating the estimated paths to the locations of the users, scatterers, and the RSU. Proposed channel estimation methods include Distributed Compressed Sensing-Simultaneous Orthogonal Matching Pursuit (DCS-SOMP) \cite{Talvitie2019}, subspace-based algorithms like multidimensional estimation via rotational invariance techniques (MD-ESPRIT) \cite{Jiang2021}, and Bayesian learning \cite{Zhu2019}, etc. The vehicle location can then be obtained through path geometric transformations \cite{Jiang2021} or probability models\cite{Talvitie2019, Zhu2019}. Some other methods more focus on location tracking \cite{ge2022mmwave, kim2022pmbm,  ge2022computationally, chu2021vehicle, chu2022joint, ruble2018wireless, mendrzik2019enabling, Wymeersch2018, mostafavi2020vehicular, gante2020deep} so that the historical channel and location information can be leveraged. Location tracking solutions or the state inference models are the focus of these papers with few mentions of channel estimation methods. Channel \ac{SLAM} techniques \cite{ge2022mmwave, kim2022pmbm,  ge2022computationally, chu2021vehicle, chu2022joint, ruble2018wireless, mendrzik2019enabling, Wymeersch2018} are a significant category of solutions for determining both the positions of scatterers and the vehicle. \ac{SLAM} filters are the primary contributions of the papers, where Poisson multi-Bernoulli mixture (PMBM) based \ac{SLAM} filters are proposed in \cite{kim2022pmbm, ge2022computationally}, and particle filter based methods are suggested in \cite{chu2021vehicle, chu2022joint, ruble2018wireless}. In \cite{mendrzik2019enabling, Wymeersch2018}, factor graphs are adopted for belief propagation and calculate the posteriors of the locations under a given channel status. An extended Kalman filter (EKF) method is implemented in \cite{mostafavi2020vehicular}. A data-driven approach is also feasible, as proposed in \cite{ gante2020deep} that builds a \ac{LSTM} and a \ac{TCN} network to extract the temporal features from the sequential power delay profiles and predict the user location. In short, the limitations shared across the prior work subject but are not limited to 1) considering oversimplified communication models which assume all digital architectures and perfect TX-RX synchronizations to exploit \ac{ToA} instead of \ac{TDoA}, and neglect the filtering effects at the transceiver; 2) using artificially controlled channels and simple simulation environment (3 - 4 reflectors instead of realistic channels with numerous uncertainties and limitations. The \ac{LOS} and first order \ac{NLOS} paths are guaranteed while higher order NLOS paths are missing, resulting in the absence of strategies to classify the reflection orders. In addition, noises are manually added to the channel parameters following statistics of channel estimation errors \cite{blanco2019performance}, which results in 3) lack of solutions for the high complexity issue brought by 3D high resolution channel estimations using the state-of-the-art compressive channel estimation strategies.  4) Unsatisfactory localization accuracy (3.g., $7.5\sim 16$ m  \cite{gante2020deep}) using simulated realistic channels is far away from the sub-meter accuracy. 





==> Sections_old/simulation_results.tex <==
\section{Simulation Results}\label{sec:SimResults}
In this section, we present simulation results to verify the concepts discussed in this work. We begin by detailing the simulation setups in Sec. \ref{Simulation setups}. Then in Sec. \ref{chanest_results}, we implement the MOMP based channel estimation to establish a solid foundation for the subsequent tasks. In Sec. \ref{PathNet_result}, we demonstrate the results of path classification using \textit{PathNet} for the simulated channels, achieving $99\%$ classification accuracy. We then discuss the localization through geometric transformations using the estimated channel parameters and predicted path orders in Sec. \ref{ini_loc_results}, where we observe that the sub-meter accuracy is not achieved for a sufficient number of users. The localization refinement using \textit{ChanFormer} is thus implemented in Sec. \ref{refined_loc_results}, which results in a considerable decrease in 2D localization errors, achieving the desired sub-meter localization.

\begin{figure}[t!]
	\centering
	\includegraphics[width=.9\columnwidth]{Figs/Sim_Env.pdf}
	\caption{Ray-tracing simulation of an urban environment with cars and trucks distributed across $4$ lanes. }
	\label{Sim_Env}
\end{figure}
\subsection{Simulation setups}\label{Simulation setups}
\textbf{Ray-tracing simulation for realistic channels: }We run $2500$ electromagnetic simulations of a vehicular environment in Rosslyn City, Virginia, on a $240\times120$ m$^2$ plane, using \textit{Wireless Insite} software\cite{WirelessInsiteSW}, as the snapshot shown in Fig. \ref{Sim_Env}. In each simulation, around $30$ vehicles are randomly distributed across the four lanes for initial access, with $80\%$ being cars and $20\%$ being trucks according to the 3GPP vehicular communication requirement \cite{3GPPVehEnv}. The RSU is located at $\bx_{\rmt}=[120, -21, 5]$ m, down facing the road. Parameters for materials of the building/territorial surfaces, the vehicle sizes, placements of antennas on the vehicle and RSU, etc., follow the deployments in \cite{anum2020passive}. $4$ active cars are randomly selected to communicate with the RSU in the $73$ GHz band. With each car equipped with $4$ communication arrays, the simulations provide $4\times 4\times 2500=40$k as the dataset $\mathcal{S}$, and every channel has $L=25$ multipath components. The first $24$k channels are split into $3:1$ for training and validations, denoted as $\mathcal{S}_{\rm tr}$ and $\mathcal{S}_{\rm val}$, and the remaining $16$k channels serve as the testing set $\mathcal{S}_{\rm te}$ for all the performance evaluations. 

\textbf{Communication system:} Localization performance with various antenna settings and transmitted power levels are studied in \cite{SAM2022}. In this paper, we use an antenna setting of $N_{\rmt} = N_{\rmt}^{\rmx}\times N_{\rmt}^{\rmy} = 16\times 16$, $N_{\rmr} = N_{\rmr}^{\rmx}\times N_{\rmr}^{\rmy} = 8\times 8$, and a transmitted power of $P_{\rmt}=40$ dBm for a better performance. The number of RF chains are set to be $N_{\rmt}^{\rm RF}=8$ and $N_{\rmr}^{\rm RF}=4$. The communication system operates at a carrier frequency $f_c=73$ GHz with a bandwidth $B_c=1$ GHz. 
$\sigma^2_{\bn}=-84$ dBm is calculated accordingly using $T=288^{\degree}$F. Given the \ac{RMS} delay-spread of the simulated channels and the bandwidth, the number of delay taps is fixed to $N_{\rmd}=64$. $N_s=\min\{N_{\rmt}^{\rm RF}, N_{\rmr}^{\rm RF}\}=4$ training data 
streams with a length of $Q=64$ are transmitted. We use the raised-cosine filter with a roll-off factor of $0.4$ as the pulse shaping function. 

\begin{figure}[b!]
	\centering
	% \column
	\subfloat[]{%
		\label{chan_est_angle_err}
		\includegraphics[width=0.9\columnwidth]{Figs/chan_est_angle_err.pdf}}\\
	\subfloat[]{%
		\label{chan_est_delay_err}
		\includegraphics[width=0.9\columnwidth]{Figs/chan_est_delay_err.pdf}}
	\caption{MOMP based channel estimation performance using a setting of a $16\times 16$ array at the TX and a $8\times 8$ array at the RX. Plots acquired based on the whole dataset $\cS$.}
	\label{chan_est_err}
\end{figure}
\subsection{MOMP based low complexity 3D channel estimation}\label{chanest_results}
% settings for MOMP channel estimation
The precoders $\bF$ are constructed by the Khatri-Rao product of the precoders along the azimuth and elevation planes, i.e., $\bF = \bF^{\rmx}\circ \bF^{\rmy}$. Each column of $\bF^{\rmx}$ ($\bF^{\rmy}$) is extracted from the DFT codebook of size $N_{\rmt}^{\rmx}$ ($N_{\rmt}^{\rmy}$), e.g., $\forall [\bF^{\rmx}]_{:,i}\in \left\{\ba'(\varphi)|\varphi=0,\frac{2\pi\cdot 1}{N_{\rmt}^{\rmx}},...,\frac{2\pi\cdot (N_{\rmt}^{\rmx}-1)}{N_{\rmt}^{\rmx}}\right\}$, where $\ba'(\varphi)=\frac{1}{\sqrt{N_{\rmt}^{\rmx}}}\left[0,e^{j\cdot 1\cdot \varphi},...,e^{j\cdot (N_{\rmt}^{\rmx}-1)\cdot \varphi}\right]^{\transp}$. The same rule applies to the combiners $\bW$. We use a setting of $M_{\rmt}=16;\ M_{\rmr}=64$, and form $\bY_M$ by collecting a total of $M=M_{\rmr}\times M_{\rmt}=1024$ frames \cite{alkhateeb2015compressed}. The size, or the resolution, of the dictionaries is based on the number of their atoms along the dimension, with a specific constant $K_{\rm res}$ determining the proportion, i.e., $N_k^{\rma}=K_{\rm res}\cdot N_k^{\rms}$. In our case, $N_1^{\rms}=N_{\rmt}^{\rmx}$, $N_2^{\rms}=N_{\rmt}^{\rmy}$, and $N_3^{\rms}=N_{\rmd}$. The impact of $K_{\rm res}$ is studied in \cite{MOMP2022}. Here we set $K_{\rm res}=128$ as it brings a comparable performance to using a higher resolution setting, such as $K_{\rm res}=1024$, while being computationally more efficient. 

The angle and delay estimation performance can be found in Fig. \ref{chan_est_err}. The estimation errors are calculated by matching an estimated path to its closest true path in the channel. We obtain better DoD estimations angle errors of $\leq 10^{\degree}$ compared to DoA estimations which mostly have angle errors of $\leq 15^{\degree}$. This is reasonable as the TX is equipped with a $16\times 16$ antenna array, while the RX array size is $8\times 8$. A delay error of $\leq 5e-8$ s can be expected. The angle and delay estimates may not appear accurate enough for localization when all estimated paths, including those with large noises such as higher order reflections, are associated with true paths. However, this does not necessarily reflect the localization accuracy as \textit{PathNet} will identify the usable paths.

\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{Figs/database_stat.pdf}
	\caption{Distribution of the power gap $\Delta|\alpha|^2$ between the LOS and strongest 1st order path of $14$k valid LOS channels from the entire dataset containing $40$k channels. $40\%$ channels are with $\Delta|\alpha|^2>30$ dB.}
	\label{database_stat}
\end{figure}


\subsection{\textit{PathNet} for path classification}\label{PathNet_result}
\textit{PathNet} is trained based on $\mathcal{S}_{\rm tr}$ and $\mathcal{S}_{\rm val}$, which lasts for $1000$ epochs with an early stopping depending on the convergence of the validation loss. We adopt Adam optimizer \cite{kingma2014adam}, and set the learning rate $1e-3$ with a decay rate of $0.95$ every $200$ training epochs. The customized weight for tweaking the penalty in $\mathcal{L}({\boldsymbol\mu})$ is set to $\eta=0.2$. The path classification performance presented in Table \ref{path_class_perform} is evaluated using the channels in $\mathcal{S}_{\rm te}$ that the network has never seen, providing classification accuracies in the order of $99\%$ in a vehicular setting, which demonstrates the strong generalization ability of the proposed simple yet effective network.
\begin{table}[h!]
	\centering
	\resizebox{.9\columnwidth}{!}{
		\begin{tabular}{lp{0.24\columnwidth}p{0.24\columnwidth}p{0.24\columnwidth}}
			\toprule
			\textbf{Overall}   & \textbf{LOS} ($c=1$)      & \textbf{1st order path} ($c=2$) & \textbf{Other} ($c=3$)    \\
			\midrule
			$98.81\%$ & $99.86\%$ & $99.13\%$             & $98.67\%$ \\
			\bottomrule
		\end{tabular}
	}
	\caption{Categorical path classification accuracy based on $16$k testing channels ($25$ paths simulated for each channel).}
	\label{path_class_perform}
\end{table}
\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{Figs/CDF_ini_perform_3D.pdf}
	\caption{Localization performance using geometric transformations based on $2349$ qualified estimated channels ($2210$ LOS; $139$ NLOS) in $\mathcal{S}^+_{\rm te}$.
	}
	\label{ini_perform}
\end{figure}
\begin{table}[b]
	\centering
	\resizebox{\columnwidth}{!}{
		\begin{tabular}{lllll}
			\toprule
			% colors: FFF0C8
			\textbf{Channel}                  & \textbf{$5$th}  & \textbf{$50$th} & \textbf{$80$th} & \textbf{$95$th} \\ \midrule
			Overall            & $0.06$ & $0.51$ & $0.92$ & $1.70$ \\ 
			\rowcolor[HTML]{FFF6CC} 
			Overall$^{\star}$  & $0.04$ & $0.22$ {\color{red} \scriptsize $57\%\downarrow$} & $0.32$ {\color{red} \scriptsize $65\%\downarrow$} &  $0.72$ {\color{red} \scriptsize $58\%\downarrow$} \\ \hline
			LOS+NLOS           & $0.06$ & $0.49$ & $0.88$ & $1.26$ \\
			\rowcolor[HTML]{FFF6CC} 
			LOS+NLOS$^{\star}$ & $0.04$ & $0.21$ {\color{red} \scriptsize $57\%\downarrow$} & $0.31$ {\color{red} \scriptsize $65\%\downarrow$} & $0.45$ {\color{red} \scriptsize $64\%\downarrow$} \\\hline
			NLOS               & $0.21$ & $1.67$ & $3.87$ & $5.97$ \\
			\rowcolor[HTML]{FFF6CC} 
			NLOS$^{\star}$     & $0.09$ & $0.75$ {\color{red} \scriptsize $55\%\downarrow$} & $3.63$ & $5.80$ \\ 
			\bottomrule
		\end{tabular}
	}
	\caption{Percentile statistics of 2D localization errors (m) with and without \textit{ChanFormer}. $\star$: location estimates refined by \textit{ChanFormer}; ``Overall" shows the merged localization results of using channels in $\mathcal{S}^+_{\rm te}$. }
	\label{all_perform}
\end{table}


\subsection{Localization based on geometric transformations}\label{ini_loc_results}
To acquire reasonable localization results, we first examine the entire database which contains $14$k valid LOS channels ($L_{c=2}\geq 1$) and $24$k valid NLOS channels ($L_{c=2}\geq 3$), and establish criteria to exclude channels indicating the vehicle being not locatable. For valid LOS channels, we measure the power gap $\Delta |\alpha|^2$ between the LOS and the strongest 1st order path, as shown in Fig. \ref{database_stat}, $40\%$ of the channels are with $\Delta |\alpha|^2>30$ dB, so the 1st order reflections cannot be estimated accurately or even detected. For valid NLOS channels, we check the received power levels to determine a threshold to ensure reliable channel estimations. It is important to note that while these simulated realistic channels provide a useful representation of real-world channels, they do have limitations due to the absence of factors such as traffic lights and building windows that can produce additional reflections, some of which can be quite strong. These factors could have an impact on the overall channel characteristics. In our settings, we argue that a vehicle is locatable when the channel status satisfies the following rules: 1) The channel is valid with sufficient paths for localization; 2) $\Delta |\alpha|^2 \leq 30$ dB for LOS channels; 3) For each NLOS-only channel, the set of 1st order reflections with a received power of $P_{\rmr}\geq -80$ dBm -- $\mathcal{Z}=\left\{\hat{\bz}_l\ |\ P_{\rmr}(l)\geq -80\ {\text{dBm}}, c(\hat{\bz}_l)=2\right\}$ -- has a length of $|\mathcal{Z}|\geq 3$. It is worth noticing that the statistic is based on ideal channels rather than the estimated, hence there are likely fewer estimated channels that qualify for usage in our localization strategy.

Considering real applications, the vehicle location is calculated based on the array with the strongest received power, thereby the dataset size is $4\times$ smaller. The new sets are denoted as $\mathcal{S}^{+}_{\rm tr}\in \mathcal{S}_{\rm tr}$, $\mathcal{S}^{+}_{\rm val}\in \mathcal{S}_{\rm val}$, and $\mathcal{S}^{+}_{\rm te}\in \mathcal{S}_{\rm te}$. There exist $2349$ qualified estimated channels ($2210$ LOS and $139$ NLOS) in $\mathcal{S}^{+}_{\rm te}$, based on which the localization performance is plotted in Fig. \ref{ini_perform}, showing the \ac{CDF} of localization error (m). The 3D error distribution is close to the 2D one, because we have the height information which helps in identifying accurate location estimates. For the following evaluations, we will primarily focus on the 2D errors. The 5, 50, 80, 95th-percentile accuracies are presented in Table \ref{all_perform}. Hereby we claim that sub-meter accuracy localization is realized for $80\%$ of the users in LOS channels and $35\%$ of the users in NLOS channels. The performance is compromised for NLOS channels because of the small pool of qualified estimated paths and the decreased accuracy of channel estimations. Nevertheless, the performance we have achieved should be considered as the worst-case scenario, as the real-world channels are likely to include more reflections from traffic lights and building windows with higher power.

\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{Figs/perform_various_tiles.pdf}
	\caption{Overall 2D localization error (m) when training \textit{ChanFormer} on $\mathcal{S}^{+}_{\rm tr}$ using various tile settings.}
	\label{perform_various_tiles}
\end{figure}
\begin{figure}[t!]
	\centering
	\includegraphics[width=\columnwidth]{Figs/CDF_ChanFormer_refined.pdf}
	\caption{\textit{ChanFormer} refined (with $^{\star}$) location estimates. The 95th-percentile 2D error is reduced by $1$ m ($58\%\downarrow$) overall. The error is $64\%\downarrow$ for $95\%$ of users in LOS channels, and $55\%\downarrow$ for $50\%$ of users in NLOS channels, realizing the expected sub-meter localization.
	}
	\label{ChanFormer_refined}
\end{figure}
\begin{figure*}[t!]
	\centering
	% \column
	\subfloat[\textbf{LOS} channel]{%
		\label{2_LOS_WI}
		\includegraphics[height=0.29\textwidth]{Figs/2_LOS_WI.pdf}}\hfill
	\subfloat[True $\bP(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})$ \textbf{(LOS)}]{%
		\label{2_LOS_True}
		\includegraphics[height=0.295\textwidth]{Figs/2_LOS_True.pdf}}
	\subfloat[Predicted $\bP(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})^{\star}$ \textbf{(LOS)}]{%
		\label{2_LOS_Pred}
		\includegraphics[height=0.295\textwidth]{Figs/2_LOS_Pred.pdf}}
	
	\subfloat[\textbf{NLOS} channel]{%
		\label{12_NLOS_WI}
		\includegraphics[height=0.29\textwidth]{Figs/12_NLOS_WI.pdf}}\hfill
	\subfloat[True $\bP(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})$ \textbf{(NLOS)}]{%
		\label{12_NLOS_True}
		\includegraphics[height=0.295\textwidth]{Figs/12_NLOS_True.pdf}}
	\subfloat[Predicted $\bP(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})^{\star}$ \textbf{(NLOS)}]{%
		\label{12_NLOS_Pred}
		\includegraphics[height=0.295\textwidth]{Figs/12_NLOS_Pred.pdf}}
	\caption{
		An example of pairs of a ground truth and a \textit{ChanFormer} predicted (with $\star$) probability map under LOS (a, b) / NLOS (c, d) conditions. (a, b) True location: $[98.07, -1.75]$; Initial error $0.50$ m; Error after refinement: $0.07$ m ($0.43$ m $\downarrow$). (c, d) True location: $[135.48, -7.75]$; Initial error: $0.56$ m; Error after refinement: $0.08$ m ($0.47$ m $\downarrow$). The examples are from $\cS_{\rm te}^+$. %{\color{red} (good examples of LOS and a NLOS cases)}
	}
	\label{prob_maps}
\end{figure*}
\begin{figure*}[t!]
	\centering
	% \column
	\subfloat[\textbf{NLOS} channel]{%
		\label{28_NLOS_WI}
		\includegraphics[height=0.29\textwidth]{Figs/28_NLOS_WI.pdf}}\hfill
	\subfloat[True $\bP(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})$ \textbf{(NLOS)}]{%
		\label{28_NLOS_True_Bad}
		\includegraphics[height=0.295\textwidth]{Figs/28_NLOS_True_Bad.pdf}}
	\subfloat[Predicted $\bP(\hat{\bZ}, \hat{\bx}_{\rmr}^{\shortparallel})^{\star}$ \textbf{(NLOS)}]{%
		\label{28_NLOS_Pred_Bad}
		\includegraphics[height=0.295\textwidth]{Figs/28_NLOS_Pred_Bad.pdf}}
	\caption{An example of a pair of true and predicted probability map when the initial estimate is far from the true location. \textit{ChanFormer} pulls the initial estimate $[115.19, -9.63]$ towards the true location $[113.55, -7.75]$, providing an error reduction from $2.5$ m to $1.36$ m ($1.13$ m $\downarrow$). 
		%{\color{red} (added a situation beyond the network's capability.)}
	}
	\label{bad_refine_case}
\end{figure*}
%\begin{table*}[t!]
%	\centering
%	\resizebox{.95\textwidth}{!}{
%		\begin{tabular}{lp{0.07\textwidth}p{0.1\textwidth}p{0.1\textwidth}p{0.13\textwidth}p{0.1\textwidth}p{0.1\textwidth}p{0.16\textwidth}}
%			\toprule
%			\textbf{Method}     & \textbf{3D}& $f_c$                                 & $B_c$ & \textbf{Array size }                            & \textbf{Realistic channels }& \textbf{Agnostic path orders} & \textbf{Error (m)}                                                          \\
%			\midrule
%			LOS / NLOS \cite{mendrzik2018harnessing} & $\times$             & $38$ GHz  & $125$ MHz       & $1\times 25$ (ULA)           & $\times$                & $\times$            & \begin{tabular}[c]{@{}l@{}}LOS: $0.016$ (PEB); \\ NLOS: $0.222$ (PEB)\end{tabular}    \\
%			
%			LOS  \cite{abu2018error}       & $\checkmark$             & $38$ GHz           & $125$ MHz       & $12\times 12$              & N/A                & $\times$             & $0.3$ (PEB)                                                                       \\
%			
%			\rowcolor[HTML]{FFF6CC} 
%			LOS / NLOS (Ours)   & $\checkmark$             & $73$ GHz                                                & $1$ GHz         & \begin{tabular}[c]{@{}l@{}}TX: $16\times 16$; \\ RX: $8\times 8$ \end{tabular} & $\checkmark$                & $\checkmark$            & \begin{tabular}[c]{@{}l@{}}LOS: $0.45$ (PEB);\\ NLOS: $0.75$ (Mean)
%			\end{tabular}\\
%			\bottomrule
%		\end{tabular}
%		
%	}
%	\caption{Comparisons with papers for error bound analysis {\color{red} (or do we also put on results from prior work?)}}.
%	\label{result_comp}
%\end{table*}

\subsection{\textit{ChanFormer} for localization refinement}\label{refined_loc_results}
The impacts of $\gamma$ and $\delta$ are studied as shown in Fig. \ref{distance_prob_model}, accordingly to which $\gamma=5$ and $\delta=1$ are set in Equ. (\ref{dist_prob_model}) to have a smooth and balanced probability function. A $5\times 5$ tile structure with a grid size $g_s=0.4 \text{ m}$ is adopted, which is found to be the best option among the settings shown in Fig. \ref{perform_various_tiles}. \textit{ChanFormer} is trained based on $3568$ qualified channels ($3316$ LOS / $252$ NLOS) in $\mathcal{S}^{+}_{\rm tr}$ and $\mathcal{S}^{+}_{\rm val}$, with a batch size of $32$. Adam optimizer is used, and  the learning rate is $2e-4$ with a decay rate of $0.95$ per $200$ epochs. Loss on the validation set is monitored for early stopping.

The refined localization performance based on set $\mathcal{S^+_{\rm te}}$ can be found in Fig. \ref{ChanFormer_refined}, and the percentile statistics are shown in Table \ref{all_perform}. Overall, the 80, 95th-percentile accuracy is improved by $65\%$ and $58\%$. The refinement reduces the 95th-percentile 2D error to $0.45$ m from $1.26$ m, i.e., $64\%$ improvement in the accuracy, for users in the LOS, and an error reduction to $0.75$ m from $1.67$ m, i.e., $55\%$ accuracy improvement, is achieved for half of the users in the channel of NLOS. In conclusion, sub-meter localization is realized for $95\%$ of the users in LOS channels and $50\%$ of the users in the channel of NLOS. Fig. \ref{prob_maps} shows an example of pairs of ground truth and predicted probability maps under LOS and NLOS situations for intuition. A reduction of 2D error from $\epsilon(\hat{\bx}_{\rmr}^{\shortparallel})=0.5 \text{ m}$ to $\epsilon(\widetilde{\bx}_{\rmr}^{\shortparallel})=0.07$ m for the LOS case, and an error reduction from $0.56$ m to $0.08$ m for the NLOS case, are realized. Note that, \textit{ChanFormer} working like a filter can be effective when the initial location estimate error $\epsilon(\hat{\bx}_{\rmr}^{\shortparallel})< 2.5$ m, allowing the network to remove the noise embedded in both $\hat{\bZ}$ and $\hat{\bx}_{\rmr}^{\shortparallel}$, and pull the location estimate in the right direction, whereas it cannot effectively correct $\epsilon(\hat{\bx}_{\rmr}^{\shortparallel})$ when $\hat{\bx}_{\rmr}^{\shortparallel}$ is hopped too far away from the tile panel, especially in the NLOS case. Fig. \ref{bad_refine_case} illustrates the situation where \textit{ChanFormer} enables an error reduction of $1.13$ m, but the error remains at $1.3$ m as the initial estimate is $2.5$ m away from the true location. 

\begin{figure}[t!]
	\centering
	\includegraphics[width=.85\columnwidth]{Figs/CDF_comp_baseline_new.pdf}
	\caption{ Comparison of joint localization and communication schemes (CDF acquired based on $\mathcal{S}^{+}_{\rm te}$ following our experimental settings). \yuncommentY{The references: MFFN \cite{lv2022deep}; \ac{CNN} using \ac{PDP} \cite{gante2020deep} will be updated once the citation index are fixed.}}
	\label{CDF_comp_baseline}
\end{figure}
Most of the previous studies mentioned in Sec. \ref{PriorWork} assume unrealistic artificially controlled channels and simplistic communication system settings, limiting their comparability to our methods. For fair comparisons, we migrated the methods in \cite{lv2022deep, gante2020deep} to our simulation environment as the two are based on realistic ray-tracing channels. We apply our channel estimation scheme to get the estimated channel parameters for the network proposed in \cite{lv2022deep}, instead of using the ideal channel parameters as considered in \cite{lv2022deep}. The reproduced localization results with our experimental settings could be found in Fig. \ref{CDF_comp_baseline}. Our model and data-driven localization method outperforms their work by achieving the sub-meter localization for $95\%$ of the users.
%{\color{red} Comparisons based on ... are shown in Table \ref{result_comp}.}



==> Sections_old/system_model.tex <==
\section{System model}\label{sec:sys_model}
%% Communication environment, illustrative figures,etc.
We consider a vehicular environment depicted in Fig. \ref{fig_cartoon_env}, where active cars are communicating with the \ac{RSU}. The RSU is equipped with a single \ac{URA}, and each car is equipped with $4$ URAs facing front, back, right, and left, as suggested in 3GPP \cite{3GPPVehEnv}. We focus on the initial access between a car and the RSU, seeking to realize sub-meter vehicle localization accuracies as a byproduct of the link establishment.
\begin{figure}[t!]
	\centering
	% \column
	\subfloat[]{%
		\label{fig_cartoon_env}
		\includegraphics[width=.95\columnwidth]{Figs/fig_cartoon_env.png}}\\
	\subfloat[]{%
		\label{Car_with_array}
		\includegraphics[height=0.4\columnwidth]{Figs/Car_with_array.pdf}}\hfill
		\subfloat[]{%
		\label{high_order_paths}
		\includegraphics[height=0.44\columnwidth]{Figs/high_order_paths.png}}
	\caption{(a) The \ac{V2I} communication environment. (b) Every car is equipped with $4$ URAs, communicating with the RSU with a single URA. (c) An example \ac{V2I} channel containing several high order reflections.}
	\label{model_cartoon}
\end{figure}
\begin{figure*}[b!]
    \centering
    \includegraphics[width=\textwidth]{Figs/Sys_model.pdf}
    \caption{Diagram of the joint initial access and localization system model. }
    \label{Sys_model}
\end{figure*}
%% Sub-section: Communication system model
\subsection{Communication system model}
We consider the downlink of a mmWave \ac{MIMO} communication system with hybrid analog-digital precoding and combining. The URA on the RSU is equipped with $N_{\rmt}=N_{\rmt}^{\rmx}\times N_{\rmt}^{\rmy}$ antenna elements and $N_{\rmt}^{\rm RF}$ RF-chains, and each URA on the vehicle has $N_{\rmr}=N_{\rmr}^{\rmx}\times N_{\rmr}^{\rmy}$ antenna elements and $N_{\rmr}^{\rm RF}$ RF-chains. We target at time-domain channel estimations as delays are required for localization. Assuming $N_s\leq \min\{N_{\rmt}^{\rm RF}, N_{\rmr}^{\rm RF}\}$ data-streams are transmitted, the hybrid precoder used at the \ac{TX} uses is defined as ${\bf F}=\bF_{\rm RF}\bF_{\rm BB}\in\mathbb{C}^{N_{\rmt}\times N_s}$, and the hybrid combiner at the \ac{RX} is ${\bW}=\bW_{\rm RF}\bW_{\rm BB}\in\mathbb{C}^{N_{\rmr}\times N_s}$. Among several RF precoder and combiner architectures, a fully connected phase shifting network \cite{mendez2016hybrid} is adopted. Training signals are transmitted using several pairs of $\bF$ and $\bW$ to sound the channel and localize a vehicle. The $q$-th instance of the training symbols is a vector denoted as $\bs[q]\in \mathbb{C}^{N_s\times 1}, q=1,...,Q$, satisfying $\mathbb{E}[\bs[q]\bs[q]^*]=\frac{1}{N_s}\bI_{N_s}$. We treat the ${N_{\rmr}\times N_{\rmt}}$ mmWave MIMO channel matrix to be frequency-selective with $N_{\rmd}$ delay taps, i.e., the channel for the $n$-th delay tap is $\bH_n\in\mathbb{C}^{N_{\rmr}\times N_{\rmt}},\ n=0,...,N_{\rmd}-1$. With a transmitted power of $P_{\rmt}$, the $q$-th instance of the received signals can be written as:
\begin{equation}\label{receive_sig}
\by[q]=\bW^*\sum\limits_{n=0}^{N_{\rmd}-1}\sqrt{P_{\rmt}}\bH_n\bF\bs[q-n]+\bW^*\bn[q],
\end{equation}
where $\bn[q]\sim \mathcal{N}({\bf 0},\sigma_{\bn}^2\bI_{N_s})$ are the additive Gaussian noise samples. We use the thermal noise $\sigma^2_{\bn}=K_{\rmB}TB_c$, where $B_c$ is the system bandwidth, for simulations. 

Note that $\mathbb{E}[\bW^*\bn[q]\bn[q]^*\bW]=\sigma_{\bn}^2\mathbb{E}[\bW^*\bW]\neq \bI$, meaning the noises at the RX are no longer white. To whiten the signal in Equ. (\ref{receive_sig}), $\by[q]$ is multiplied by the inverse of a lower triangular matrix $\bL$ as $\breve{\by}[q]=\bL^{-1}\by[q]$, where $\bL$ is acquired by the Cholesky decomposition $\bW^*\bW=\bL\bL^*$.  Let $\breve{\bW}=\bL^{-1}\bW$ and $\breve{\bn}[q]=\bL^{-1}\bW^*\bn[q]$, Equ. (\ref{receive_sig}) can be rewritten as:
\begin{equation}\label{whietened_receive_sig}
    \breve{\by}[q]=\breve{\bW}^*\sum\limits_{n=0}^{N_{\rmd}-1}\sqrt{P_{\rmt}}\bH_n\bF\bs[q-n]+\breve{\bn}[q],
\end{equation}
and accordingly $\mathbb{E}[\breve{\bn}[q]\breve{\bn}[q]^*]=\sigma_{\bn}^2\mathbb{E}[\bL^{-1}\bW^*\bW(\bL^{-1})^{*}]= \sigma_{\bn}^2\bI$.  Let $\breve{\bY}=[\breve{\by} [1],...,\breve{\by} [Q]]\in \mathbb{C}^{N_s\times Q}$ be the matrix collecting the received signals, and $\breve{\bN} =[\breve{\bn} [1],...,\breve{\bn} [Q]]$ be the noise matrix, Equ. (\ref{whietened_receive_sig}) can be extended to:
\begin{equation}\label{receive_mat}
\breve{\bY} =\breve{\bW}^* [\bH_0,...,\bH_{N_{\rmd}-1}]\left((\bI_{N_{\rmd}}\otimes\bF )\bS \right)+\breve{\bN},
\end{equation}
where 
\begin{equation}
    \bS=
    \begin{bmatrix} \bs[1] & \bs[2] & \hdots & \bs[Q] \\ 
    {\bf 0} & \bs[1] & \hdots & \bs[Q-1] \\ 
    \vdots & \vdots & \ddots  & \vdots \\
    {\bf 0}  & {\bf 0}&  \hdots & \bs[Q-(N_{\rmd}-1)]
    
    \end{bmatrix}.
\end{equation}
When using a set of $M_{\rmt}$ precoders $\{\bF_{m_{\rmt}}|m_{\rmt}=1,...,M_{\rmt}\}$, and a set of $M_{\rmr}$ combiners $\{\bW_{m_{\rmr}}|m_{\rmr}=1,...,M_{\rmr}\}$, $\breve{\bY}$ becomes $\breve{\bY}_{m_{\rmr}, m_{\rmt}}$ collecting the received signals with $\bF_{m_{\rmt}}$ and $\bW_{m_{\rmr}}$, and $\bS$ and $\breve{\bN}$ are changed to $\bS_{m_{\rmr}, m_{\rmt}}$ and $\breve{\bN}_{m_{\rmr}, m_{\rmt}}$ in Equ. (\ref{receive_mat}).

%% Sub-section: Communication channel model
\subsection{Communication channel model}
We consider a 3D channel model for the 3D localization purpose. $\theta^{\rmx}$ and $\theta^{\rmy}$ denote the azimuth and elevation \ac{DoA}, and $\phi^{\rmx}$ and $\phi^{\rmy}$ represent the \ac{DoD}, as illustrated in Fig. \ref{DoD_illustration}. The unitary vector of \ac{DoA} and \ac{DoD} are accordingly given by ${\boldsymbol \theta}=[\cos\theta^{\rmy}\cos\theta^{\rmx}, \cos\theta^{\rmy}\sin\theta^{\rmx}, \sin\theta^{\rmy}]^{\transp}$ , and DoD ${\boldsymbol \phi}=[\cos\phi^{\rmy}\cos\phi^{\rmx}, \cos\phi^{\rmy}\sin\phi^{\rmx}, \sin\phi^{\rmy}]^{\transp}$, which are employed for simpler computations in our localization scheme. The array responses at the TX and RX are $\ba_{\rmt}({\boldsymbol\phi})=\ba(\phi^{\rmx})\otimes \ba(\phi^{\rmy})$ and $\ba_{\rmr}({\boldsymbol\theta})=\ba(\theta^{\rmx})\otimes \ba(\theta^{\rmy})$, where $\ba(\phi^{\rmx})\in \mathbb{C}^{N_{\rmt}^{\rmx}\times 1}$ ($\ba(\phi^{\rmy})\in \mathbb{C}^{N_{\rmt}^{\rmy}\times 1}$) is the steering vector along the dimension:
\begin{equation}
    \ba(\phi^{\rmx})=\left[1,e^{-j2\pi\vartheta^{\rmx}\sin(\phi^{\rmx})},...,e^{-j(N^{\rmx}_{\rmt}-1)2\pi\vartheta^{\rmx}\sin(\phi^{\rmx})}\right]^{\transp},
\end{equation}
where $\vartheta$ is the inter-element spacing normalized by the wavelength. The steering vector at the RX $\ba_{\rmr}({\boldsymbol\theta})$ is defined similarly. The effective baseband channel is seen through the RF front end, so the effects of filter responses for band limiting -- $f_{\rmp}(t)$ which is the pulse shaping filter response evaluated at $t$ -- should be included in the channel model. As such, $\bH_n$ is formulated as:
\begin{equation}
    \bH_n=\sum\limits_{l=1}^{L}\alpha_lf_{\rmp}\left(nT_s-(t_l-t_0)\right)\ba_{\rmr}({\boldsymbol\theta}_l)\ba_{\rmt}({\boldsymbol\phi}_l)^*,
\end{equation}
where $\alpha_l$ and $t_l$ are the complex gain and the \ac{ToA} of the $l$-th path, $T_s$ is the signaling interval, and $t_0$ is the unknown clock offset.

%% Sub-section: explanation of the joint initial access and localization workflow
\subsection{Proposed joint initial access and localization}
The diagram of our proposed joint initial access and 3D vehicle localization strategy is shown in Fig. \ref{Sys_model}. First, we collect a number of measurements of mmWave received signals $\bY_M$, and implement MOMP based low complexity channel estimations to acquire $N_{\rm est}$ estimated paths $\hat{\bZ}=[\hat{\bz}_1,...,\hat{\bz}_{N_{\rm est}}]$, where each $\hat{\bz}_l$ contains the estimated channel gains $|\alpha_l|$, \ac{TDoA}s $\tau_l$, \ac{DoA}s ${\boldsymbol\theta}_l$, and \ac{DoD}s ${\boldsymbol\phi}_l$. The proposed localization strategy exploiting path geometric transformations can function in both \ac{LOS} and \ac{NLOS} channels, requiring a sufficient number of 1st order reflections. Due to the majority of the paths being higher order reflections in realistic channels, \textit{PathNet} is offered as a data-driven way to get the path orders and remove the higher order reflections. It predicts the probability of $\hat{\bz}_{l}$ being a LOS component, a 1st reflection, or a higher order reflection, and categorizes the path accordingly. A network like \textit{PathNet} could be the most effective solution for the task given the difficulty in formulating the relationship between the channel parameters and the path orders.  Following that, 3D localization based on two types of geometric transformations can be performed depending on the channel status. We observe that the initial location estimates cannot guarantee sub-meter accuracy for most of the users because of the inherent inaccuracies in the channel estimation and path classification processes.  \textit{ChanFormer} is thus proposed to analyze the relationships among the estimated paths in $\hat{\bZ}$ as well as measure the congruence between the channel features and the initial location estimate $\hat{\bx}_{\rmr}^{\shortparallel}$, and then provide a refined location estimate. The input estimated channel features are extracted through self-attention in the encoder section of the network. These features are then decoded and matched to a more accurate location estimate. The output from \textit{ChanFormer} is a probability map showing which tile contains the true location. Though we use a square tile structure in this paper, the number and the shape of the tiles could be both customized to suit the specific environment.


